Bootstrapping Inductive and Coinductive Types in HasCASL

We discuss the treatment of initial datatypes and final process types in the wide-spectrum language HasCASL. In particular, we present specifications that illustrate how datatypes and process types arise as bootstrapped concepts using HasCASL's type class mechanism, and we describe constructions of types of finite and infinite trees that establish the conservativity of datatype and process type declarations adhering to certain reasonable formats. The latter amounts to modifying known constructions from HOL to avoid unique choice; in categorical terminology, this means that we establish that quasitoposes with an internal natural numbers object support initial algebras and final coalgebras for a range of polynomial functors, thereby partially generalising corresponding results from topos theory. Moreover, we present similar constructions in categories of internal complete partial orders in quasitoposes.

==> Algebra.pp.tex <==
\SPEC \=\SIdIndex{Algebra} \Ax{=}\\
\> \SId{PolyFunctors}\\
\THEN \=\VAR \=\Id{F} \Ax{:} \Id{Functor}; \Id{a}, \Id{b} \Ax{:} \Id{Type}\\
\> \TYPE \=\Id{Alg} \Ax{:} \=\Id{Functor} \Ax{\rightarrow} \=\Id{Type} \Ax{\rightarrow} \Id{Type} \\
\>\> \Id{\Ax{:}\Ax{=}} \Ax{\lambda} \=(\Id{F} \Ax{:} \Id{Functor}) (\Id{a} \Ax{:} \Id{Type}) \Ax{\bullet} \=\Id{F} \Id{a} \Ax{\rightarrow} \Id{a}\\
\> \OP \=\Ax{\_\_}\Ax{::}\Ax{\_\_}\Ax{->}\Ax{\_\_} \Ax{:} \=\Id{Pred} (\=(\=\Id{a} \Ax{\rightarrow} \Id{b}) \Ax{\times} (\=\Id{Alg} \Id{F} \Id{a}) \Ax{\times} (\=\Id{Alg} \Id{F} \Id{b}))\\
\> \VAR \=\Id{f} \Ax{:} \=\Id{a} \Ax{\rightarrow} \Id{b}; \Id{alpha} \Ax{:} \=\Id{Alg} \Id{F} \Id{a}; \Id{beta} \Ax{:} \=\Id{Alg} \Id{F} \Id{b}\\
\> \Ax{\bullet} \=(\=\Id{f} \Ax{::} \Id{alpha} \Ax{->} \Id{beta}) \Ax{\Leftrightarrow} \\
\>\> (\=\Id{beta} \Id{comp} (\=\Id{map} \Id{f})) \Ax{=} (\=\Id{f} \Id{comp} \Id{alpha});\\
\> \TYPE \=\Id{AlgMor}\=(\Id{F} \Ax{:} \Id{Functor}) (\Id{a} \Ax{:} \Id{Type}) (\Id{b} \Ax{:} \Id{Type}) \Ax{=} \{(\=\Id{f}, \Id{alpha}, \Id{beta}) \Ax{:} (\=\Id{a} \Ax{\rightarrow} \Id{b}) \Ax{\times} \Id{Alg} \Id{F} \Id{a} \Ax{\times} \=\Id{Alg} \Id{F} \Id{b} \Ax{\bullet} \\
\>\> \Id{f} \Ax{::} \Id{alpha} \Ax{->} \Id{beta}\}\\
\> \CLASS \Id{DTFunctor} \Ax{<} \Id{Functor}\\
\> \{\VAR \=\Id{F} \Ax{:} \Id{DTFunctor}; \Id{a} \Ax{:} \Id{Type};\\
\> \TYPE \Id{InitialCarrier}(\Id{F} \Ax{:} \Id{DTFunctor});\\
\> \OP \=\Id{initialAlg} \Ax{:} \=\Id{Alg} \Id{F} (\=\Id{InitialCarrier} \Id{F});\\
\>\> \Id{fold} \Ax{:} \=\Id{Alg} \Id{F} \Id{a} \Ax{\rightarrow} \=\Id{InitialCarrier} \Id{F} \Ax{\rightarrow} \Id{a};\\
\> \VAR \=\Id{alpha} \Ax{:} \=\Id{Alg} \Id{F} \Id{a}; \Id{g} \Ax{:} \=\Id{InitialCarrier} \Id{F} \Ax{\rightarrow} \Id{a};\\
\> \Ax{\bullet} \=(\=\Id{g} \Ax{::} \Id{initialAlg} \Ax{->} \Id{alpha}) \Ax{\Leftrightarrow} \=\Id{g} \Ax{=} \=\Id{fold} \Id{alpha};;\\
\> \};\\
\> \CLASS \Id{PolyFunctor} \Ax{<} \Id{DTFunctor};\\
\> \VAR \Id{G} \Ax{:} \Id{PolyBifunctor}\\
\> \TYPE \=\Id{ParamDT} \Ax{:} \=\Id{PolyBifunctor} \Ax{\rightarrow} \=\Id{Type} \Ax{\rightarrow} \Id{Type} \\
\>\> \Id{\Ax{:}\Ax{=}} \Ax{\lambda} \=(\Id{G} \Ax{:} \Id{PolyBifunctor}) (\Id{a} \Ax{:} \Id{Type}) \Ax{\bullet} \=\Id{InitialCarrier} \\
\>\>\> (\=\Id{G} \Id{a})\\
\> \TYPE \Id{ParamDT}(\Id{G} \Ax{:} \Id{PolyBifunctor}) \Ax{:} \Id{DTFunctor}\\
\> \VAR \=\Id{l} \Ax{:} \=\Id{ParamDT} \Id{G} \Id{a}; \Id{b} \Ax{:} \Id{Type}; \Id{f} \Ax{:} \=\Id{a} \Ax{\rightarrow} \Id{b}\\
\> {\small{}\KW{\%\%}\Ax{.} map f l \Ax{=} fold initialAlg l}\\
\KW{end}

==> CTree.hascasl.pp.tex <==
\begin{hetcasl}
\KW{library} \SId{library}\\
\\
\KW{logic} \SId{HasCASL}\\
\\
\SPEC \=\SIdIndex{Dummy} \Ax{=}\\
\> \SORT \=\Id{Nat}, \Id{Tree}\\
\> \VAR \Id{a} \Ax{:} \Id{Type}\\
\> \KW{generated} \\
\> \TYPE \=\Id{CTree}(\Id{a} \Ax{:} \Id{Type}) \Ax{::=} \=\Id{leaf} \Id{a} \AltBar{} \Id{branch} (\=\Id{Nat} \Ax{\rightarrow?} \Id{Tree})\\
\KW{end}
\end{hetcasl}


==> Lambda.hascasl.pp.tex <==
\begin{hetcasl}
\KW{library} \SId{library}\\
\\
\KW{logic} \SId{HasCASL}\\
\\
\SPEC \=\SIdIndex{Dummy} \Ax{=}\\
\> \SORT \=\Id{a}, \Id{b}\\
\> \KW{free} \KW{type} \=\Id{L} \Ax{::=} \Id{abs} (\=\Id{a} \Ax{\rightarrow} \Id{b})\\
\KW{end}
\end{hetcasl}


==> RoseTree.hascasl.pp.tex <==
\begin{hetcasl}
\KW{library} \SId{library}\\
\\
\KW{logic} \SId{HasCASL}\\
\\
\SPEC \=\SIdIndex{Dummy} \Ax{=}\\
\> \VAR \Id{a}, \Id{b} \Ax{:} \Id{Type}\\
\> \TYPE \Id{Sree} \Ax{:} \=\Id{Type} \Ax{\rightarrow} \=\Id{Type} \Ax{\rightarrow} \Id{Type}\\
\> \KW{free} \KW{type} \=\Id{List} \Id{a} \Ax{::=} \=\Id{nil} \AltBar{} \Id{cons} (\=\Id{a}; \=\Id{List} \Id{a})\\
\> \KW{free} \KW{type} \=\Id{Tree} \Id{a} \Id{b} \Ax{::=} \=\Id{leaf} \Id{a} \AltBar{} \Id{branch} (\=\Id{b} \Ax{\rightarrow} \=\Id{List} (\=\Id{Sree} \Id{a} \Id{b}))\\
\KW{end}
\end{hetcasl}


==> Sys.hascasl.pp.tex <==
\begin{hetcasl}
\KW{library} \SId{library}\\
\\
\KW{logic} \SId{HasCASL}\\
\\
\SPEC \=\SIdIndex{Dummy} \Ax{=}\\
\> \VAR \Id{a}, \Id{b} \Ax{:} \Id{Type}\\
\> \TYPE \Id{SSys} \Ax{:} \=\Id{Type} \Ax{\rightarrow} \Id{Type}\\
\> \KW{generated} \TYPE \=\Id{Set}(\Id{a} \Ax{:} \Id{Type}) \Ax{::=} \=\Id{empty} \AltBar{} \Id{add} \=\Id{a} (\=\Id{Set} \Id{a})\\
\> \KW{generated} \TYPE \=\Id{Sys}(\Id{b} \Ax{:} \Id{Type}) \Ax{::=} \Id{node} \=\Id{b} (\=\Id{Set} (\=\Id{SSys} \Id{b}))\\
\KW{end}
\end{hetcasl}


==> Tree.hascasl.pp.tex <==
\begin{hetcasl}
\KW{library} \SId{library}\\
\\
\KW{logic} \SId{HasCASL}\\
\\
\SPEC \=\SIdIndex{Dummy} \Ax{=}\\
\> \VAR \Id{a}, \Id{b} \Ax{:} \Id{Type}\\
\> \TYPE \Id{Sree} \Ax{:} \=\Id{Type} \Ax{\rightarrow} \=\Id{Type} \Ax{\rightarrow} \Id{Type}\\
\> \KW{free} \KW{type} \=\Id{Tree} \Id{a} \Id{b} \Ax{::=} \=\Id{leaf} \Id{b} \AltBar{} \Id{branch} (\=\Id{a} \Ax{\rightarrow} \=\Id{Sree} \Id{a} \Id{b})\\
\KW{end}
\end{hetcasl}


==> functors.hascasl.pp.tex <==
\begin{hetcasl}
\KW{library} \SId{library}\\
\\
\KW{logic} \SId{HasCASL}\\
\\
\SPEC \=\SIdIndex{Functor} \Ax{=}\\
\> \VAR \=\Id{a}, \Id{b}, \Id{c} \Ax{:} \Id{Type}; \Id{x} \Ax{:} \Id{a}; \Id{f} \Ax{:} \=\Id{a} \Ax{\rightarrow} \Id{b}; \Id{g} \Ax{:} \=\Id{b} \Ax{\rightarrow} \Id{c}\\
\> \OP \=\Ax{\_\_}\Id{comp}\Ax{\_\_} \Ax{:} \=(\=\Id{b} \Ax{\rightarrow} \Id{c}) \Ax{\times} (\=\Id{a} \Ax{\rightarrow} \Id{b}) \Ax{\rightarrow} \=\Id{a} \Ax{\rightarrow} \Id{c};\\
\>\> \Id{id} \Ax{:} \=\Id{a} \Ax{\rightarrow} \Id{a}\\
\> \Ax{\bullet} \=\Id{id} \Id{x} \Ax{=} \Id{x}\\
\> \Ax{\bullet} \=(\=\Id{g} \Id{comp} \Id{f}) \Id{x} \Ax{=} \=\Id{g} (\=\Id{f} \Id{x});\\
\> \CLASS \Id{Functor} \Ax{<} \=\Id{Type} \Ax{\rightarrow} \Id{Type}\\
\> \{\VAR \=\Id{a}, \Id{b}, \Id{c} \Ax{:} \Id{Type}; \Id{F} \Ax{:} \Id{Functor}; \Id{f} \Ax{:} \=\Id{a} \Ax{\rightarrow} \Id{b}; \Id{g} \Ax{:} \=\Id{b} \Ax{\rightarrow} \Id{c};\\
\> \OP \=\Id{map} \Ax{:} \=(\=\Id{a} \Ax{\rightarrow} \Id{b}) \Ax{\rightarrow} \=\Id{F} \Id{a} \Ax{\rightarrow} \=\Id{F} \Id{b};\\
\> \Ax{\bullet} \=\Id{map} \Id{id} \Ax{=} (\=\Id{id} \Ax{:} \=\Id{F} \Id{a} \Ax{\rightarrow} \=\Id{F} \Id{a})\\
\> \Ax{\bullet} \=(\=\Id{map} (\=\Id{g} \Id{comp} \Id{f}) \Ax{:} \=\Id{F} \Id{a} \Ax{\rightarrow} \=\Id{F} \Id{c}) \Ax{=} \\
\>\> (\=(\=\Id{map} \Id{g}) \Id{comp} (\=\Id{map} \Id{f}));;\\
\> \};\\
\> \CLASS \Id{Bifunctor} \Ax{<} \=\Id{Type} \Ax{\rightarrow} \Id{Functor}\\
\> \{\VAR \=\Id{a}, \Id{b}, \Id{c}, \Id{d} \Ax{:} \Id{Type}; \Id{F} \Ax{:} \Id{Bifunctor}; \Id{f} \Ax{:} \=\Id{a} \Ax{\rightarrow} \Id{b}; \\
\>\> \Id{g} \Ax{:} \=\Id{b} \Ax{\rightarrow} \Id{c}; \Id{h} \Ax{:} \=\Id{c} \Ax{\rightarrow} \Id{d};\\
\> \OP \=\Id{parmap} \Ax{:} \=(\=\Id{a} \Ax{\rightarrow} \Id{b}) \Ax{\rightarrow} \=\Id{F} \Id{a} \Id{d} \Ax{\rightarrow} \=\Id{F} \Id{b} \Id{d};\\
\> \Ax{\bullet} \=\Id{parmap} \Id{id} \Ax{=} (\=\Id{id} \Ax{:} \=\Id{F} \Id{a} \Id{d} \Ax{\rightarrow} \=\Id{F} \Id{a} \Id{d})\\
\> \Ax{\bullet} \=(\=\Id{parmap} (\=\Id{g} \Id{comp} \Id{f}) \Ax{:} \=\Id{F} \Id{a} \Id{d} \Ax{\rightarrow} \=\Id{F} \Id{c} \Id{d}) \Ax{=} \\
\>\> (\=(\=\Id{parmap} \Id{g}) \Id{comp} (\=\Id{parmap} \Id{f}));;\\
\> \};\\
\> \Ax{\bullet} \=(\=(\=\Id{parmap} \Id{f}) \Id{comp} (\=\Id{map} \Id{h}) \Ax{:} \=\Id{F} \Id{a} \Id{c} \Ax{\rightarrow} \=\Id{F} \Id{b} \Id{d}) \Ax{=} \\
\>\> (\=(\=\Id{map} \Id{h}) \Id{comp} (\=\Id{parmap} \Id{f}));\\
\KW{end}\\
\\
\SPEC \=\SIdIndex{PolyFunctors} \Ax{=}\\
\> \SId{Functor}\\
\THEN \=\CLASS \Id{PolyFunctor} \Ax{<} \Id{Functor};\\
\> \VAR \=\Id{F}, \Id{G} \Ax{:} \Id{PolyFunctor}; \Id{a}, \Id{b} \Ax{:} \Id{Type}\\
\> \TYPE \Id{Const}(\Id{a} \Ax{:} \Id{Type}), \Id{Id}, \\
\> \Id{Sum}\=(\Id{F} \Ax{:} \Id{PolyFunctor}) (\Id{G} \Ax{:} \Id{PolyFunctor}), \\
\> \Id{Prod}\=(\Id{F} \Ax{:} \Id{PolyFunctor}) (\Id{G} \Ax{:} \Id{PolyFunctor}), \\
\> \Id{Exp}\=(\Id{F} \Ax{:} \Id{PolyFunctor}) (\Id{a} \Ax{:} \Id{Type}) \Ax{:} \Id{PolyFunctor}\\
\> \TYPE \=\Id{Const}\=(\Id{a} \Ax{:} \Id{Type}) (\Id{b} \Ax{:} \Id{Type}) \Ax{::=} \Id{mkConst} (\Id{getConst} \Ax{:} \Id{a})\\
\> \TYPE \=\Id{Id}(\Id{b} \Ax{:} \Id{Type}) \Ax{::=} \Id{mkId} (\Id{getId} \Ax{:} \Id{b})\\
\> \TYPE \=\Id{Sum}\=(\Id{F} \Ax{:} \Id{PolyFunctor}) (\Id{G} \Ax{:} \Id{PolyFunctor}) (\Id{b} \Ax{:} \Id{Type}) \\
\>\> \Ax{::=} \=\Id{inl} (\=\Id{F} \Id{b}) \AltBar{} \Id{inr} (\=\Id{G} \Id{b})\\
\> \VAR \=\Id{f} \Ax{:} \=\Id{F} \Id{b} \Ax{\rightarrow?} \Id{a}; \Id{g} \Ax{:} \=\Id{G} \Id{b} \Ax{\rightarrow?} \Id{a}; \Id{h} \Ax{:} \=\Id{Sum} \Id{F} \Id{G} \Id{b} \Ax{\rightarrow?} \Id{a}\\
\> \OP \=\Id{sumcase} \Ax{:} \=(\=\Id{F} \Id{b} \Ax{\rightarrow?} \Id{a}) \Ax{\rightarrow} \=(\=\Id{G} \Id{b} \Ax{\rightarrow?} \Id{a}) \Ax{\rightarrow} \=(\=\Id{Sum} \Id{F} \Id{G}) \Id{b} \Ax{\rightarrow?} \Id{a}\\
\> \Ax{\bullet} \=\Id{h} \Ax{=} \=\Id{sumcase} \Id{f} \Id{g} \Ax{\Leftrightarrow} \\
\>\> (\=\Ax{\forall} \Id{x} \Ax{:} \=\Id{F} \Id{b}; \Id{y} \Ax{:} \=\Id{G} \Id{b} \Ax{\bullet} \=\Id{h} (\=\Id{inl} \Id{x}) \Ax{=} \=\Id{f} \Id{x} \Ax{\wedge} \=\Id{h} (\=\Id{inr} \Id{y}) \Ax{=} \=\Id{g} \Id{y});\\
\> \TYPE \=\Id{Prod}\=(\Id{F} \Ax{:} \Id{PolyFunctor}) (\Id{G} \Ax{:} \Id{PolyFunctor}) (\Id{b} \Ax{:} \Id{Type}) \\
\>\> \Ax{::=} \Id{pair} (\=\Id{outl} \Ax{:} \=\Id{F} \Id{b}; \Id{outr}
\Ax{:} \=\Id{G} \Id{b})\\ 
\> \Ax{\bullet} \=\Ax{\forall} \Id{z} \Ax{:} \=\Id{Prod} \Id{F} \Id{G} \Id{b} \Ax{\bullet} \=\Id{z} \Ax{=} \=\Id{pair} (\=\Id{outl} \Id{z}, \=\Id{outr} \Id{z});\\
\> \TYPE \=\Id{Exp}\=(\Id{F} \Ax{:} \Id{PolyFunctor}) (\Id{a} \Ax{:} \Id{Type}) (\Id{b} \Ax{:} \Id{Type}) \\
\>\> \Ax{::=} \Id{mkExp} (\Id{getExp} \Ax{:} \=\Id{a} \Ax{\rightarrow} \=\Id{F} \Id{b})\\
\> \VAR \Id{k} \Ax{:} \=\Id{a} \Ax{\rightarrow} \Id{b}\\
\> \Ax{\bullet} \=(\=\Id{map} \Id{k} \Ax{:} \=\Id{Sum} \Id{F} \Id{G} \Id{a} \Ax{\rightarrow} \=\Id{Sum} \Id{F} \Id{G} \Id{b}) \Ax{=} \\
\>\> \Id{sumcase} (\=\Id{inl} \Id{comp} (\=\Id{map} \Id{k})) (\=\Id{inr} \Id{comp} (\=\Id{map} \Id{k}));\\
\> \CLASS \=\Id{PolyBifunctor} \Ax{<} \=\Id{Type} \Ax{\rightarrow} \Id{PolyFunctor};\\
\>\> \Id{PolyBifunctor} \Ax{<} \Id{Bifunctor};\\
\KW{end}\\
\\
\SPEC \=\SIdIndex{Algebra} \Ax{=}\\
\> \SId{PolyFunctors}\\
\THEN \=\VAR \=\Id{F} \Ax{:} \Id{Functor}; \Id{a}, \Id{b} \Ax{:} \Id{Type}\\
\> \TYPE \=\Id{Alg} \Ax{:} \=\Id{Functor} \Ax{\rightarrow} \=\Id{Type} \Ax{\rightarrow} \Id{Type} \\
\>\> \Id{\Ax{:}\Ax{=}} \Ax{\lambda} \=(\Id{F} \Ax{:} \Id{Functor}) (\Id{a} \Ax{:} \Id{Type}) \Ax{\bullet} \=\Id{F} \Id{a} \Ax{\rightarrow} \Id{a}\\
\> \OP \=\Ax{\_\_}\Ax{::}\Ax{\_\_}\Ax{->}\Ax{\_\_} \Ax{:} \=\Id{Pred} (\=(\=\Id{a} \Ax{\rightarrow} \Id{b}) \Ax{\times} (\=\Id{Alg} \Id{F} \Id{a}) \Ax{\times} (\=\Id{Alg} \Id{F} \Id{b}))\\
\> \VAR \=\Id{f} \Ax{:} \=\Id{a} \Ax{\rightarrow} \Id{b}; \Id{alpha} \Ax{:} \=\Id{Alg} \Id{F} \Id{a}; \Id{beta} \Ax{:} \=\Id{Alg} \Id{F} \Id{b}\\
\> \Ax{\bullet} \=(\=\Id{f} \Ax{::} \Id{alpha} \Ax{->} \Id{beta}) \Ax{\Leftrightarrow} \\
\>\> (\=\Id{beta} \Id{comp} (\=\Id{map} \Id{f})) \Ax{=} (\=\Id{f} \Id{comp} \Id{alpha});\\
\> \TYPE \=\Id{AlgMor}\=(\Id{F} \Ax{:} \Id{Functor}) (\Id{a} \Ax{:} \Id{Type}) (\Id{b} \Ax{:} \Id{Type}) \Ax{=} \\
\>\> \{(\=\Id{f}, \Id{alpha}, \Id{beta}) \Ax{:} (\=\Id{a} \Ax{\rightarrow} \Id{b}) \Ax{\times} \Id{Alg} \Id{F} \Id{a} \Ax{\times} \=\Id{Alg} \Id{F} \Id{b} \Ax{\bullet} \\
\>\> \Id{f} \Ax{::} \Id{alpha} \Ax{->} \Id{beta}\\
\>\> \}\\
\> \CLASS \=\Id{DTFunctor} \Ax{<} \Id{Functor};\\
\>\> \Id{PolyFunctor} \Ax{<} \Id{DTFunctor}\\
\>\> \{\VAR \=\Id{F} \Ax{:} \Id{DTFunctor}; \Id{a} \Ax{:} \Id{Type};\\
\>\> \TYPE \Id{InitialCarrier}(\Id{F} \Ax{:} \Id{DTFunctor});\\
\>\> \OP \=\Id{initialAlg} \Ax{:} \=\Id{Alg} \Id{F} (\=\Id{InitialCarrier} \Id{F});\\
\>\>\> \Id{ifold} \Ax{:} \=\Id{Alg} \Id{F} \Id{a} \Ax{\rightarrow} \=\Id{InitialCarrier} \Id{F} \Ax{\rightarrow} \Id{a};\\
\>\> \VAR \=\Id{alpha} \Ax{:} \=\Id{Alg} \Id{F} \Id{a}; \Id{g} \Ax{:} \=\Id{InitialCarrier} \Id{F} \Ax{\rightarrow} \Id{a};\\
\>\> \Ax{\bullet} \=(\=\Id{g} \Ax{::} \Id{initialAlg} \Ax{->} \Id{alpha}) \Ax{\Leftrightarrow} \=\Id{g} \Ax{=} \=\Id{ifold} \Id{alpha};;\\
\>\> \};\\
\> \VAR \Id{G} \Ax{:} \Id{PolyBifunctor}\\
\> \TYPE \=\Id{ParamDT}\=(\Id{G} \Ax{:} \Id{PolyBifunctor}) (\Id{a} \Ax{:} \Id{Type}) \\
\>\> \Ax{::=} \Id{mkPDT} (\Id{getPDT} \Ax{:} \=\Id{InitialCarrier}
(\=\Id{G} \Id{a}))\\ 
\> \Ax{\bullet} \=\Ax{\forall} \Id{l} \Ax{:} \=\Id{ParamDT} \Id{G} \Id{a} \Ax{\bullet} \=\Id{mkPDT} (\=\Id{getPDT} \Id{l}) \Ax{=} \Id{l};\\
\> \TYPE \Id{ParamDT}(\Id{G} \Ax{:} \Id{PolyBifunctor}) \Ax{:} \Id{DTFunctor}\\
\> \VAR \=\Id{l} \Ax{:} \=\Id{ParamDT} \Id{G} \Id{a}; \Id{b} \Ax{:} \Id{Type}; \Id{f} \Ax{:} \=\Id{a} \Ax{\rightarrow} \Id{b}\\
\> \Ax{\bullet} \=\Id{map} \Id{f} \Id{l} \Ax{=} \\
\>\> \Id{mkPDT} (\=\Id{ifold} (\=\Id{initialAlg} \Id{comp} (\=\Id{parmap} \Id{f})) (\=\Id{getPDT} \Id{l}));\\
\KW{end}
\end{hetcasl}


==> functors2.hascasl.pp.tex <==
\begin{hetcasl}
\KW{library} \SId{library}\\
\\
\KW{logic} \SId{HasCASL}\\
\\
\SPEC \=\SIdIndex{Functor} \Ax{=}\\
\> \VARS \=\Id{a}, \Id{b}, \Id{c} \Ax{:} \Id{Type}; \Id{x} \Ax{:} \Id{a}; \Id{f} \Ax{:} \=\Id{a} \Ax{\rightarrow} \Id{b}; \Id{g} \Ax{:} \=\Id{b} \Ax{\rightarrow} \Id{c}\\
\> \OPS \=\Ax{\_\_}\Id{comp}\Ax{\_\_} \Ax{:} \=(\=\Id{b} \Ax{\rightarrow} \Id{c}) \Ax{\times} (\=\Id{a} \Ax{\rightarrow} \Id{b}) \Ax{\rightarrow} \=\Id{a} \Ax{\rightarrow} \Id{c};\\
\>\> \Id{id} \Ax{:} \=\Id{a} \Ax{\rightarrow} \Id{a}\\
\> \Ax{\bullet} \=\Id{id} \Id{x} \Ax{=} \Id{x}\\
\> \Ax{\bullet} \=(\=\Id{g} \Id{comp} \Id{f}) \Id{x} \Ax{=} \=\Id{g} (\=\Id{f} \Id{x});\\
\> \CLASS \=\Id{Functor} \Ax{<} \=\Id{Type} \Ax{\rightarrow} \Id{Type}\\
\>\> \{\VARS \=\Id{a}, \Id{b}, \Id{c} \Ax{:} \Id{Type}; \Id{F} \Ax{:} \Id{Functor}; \Id{f} \Ax{:} \=\Id{a} \Ax{\rightarrow} \Id{b}; \Id{g} \Ax{:} \=\Id{b} \Ax{\rightarrow} \Id{c}\\
\>\> \OP \=\Id{map} \Ax{:} \=(\=\Id{a} \Ax{\rightarrow} \Id{b}) \Ax{\rightarrow} \=\Id{F} \Id{a} \Ax{\rightarrow} \=\Id{F} \Id{b}\\
\>\> \Ax{\bullet} \=\Id{map} \Id{id} \Ax{=} (\=\Id{id} \Ax{:} \=\Id{F} \Id{a} \Ax{\rightarrow} \=\Id{F} \Id{a})\\
\>\> \Ax{\bullet} \=(\=\Id{map} (\=\Id{g} \Id{comp} \Id{f}) \Ax{:} \=\Id{F} \Id{a} \Ax{\rightarrow} \=\Id{F} \Id{c}) \Ax{=} \=\Id{map} \Id{g} \Id{comp} \=\Id{map} \Id{f};\\
\>\> \}\\
\> \CLASS \=\Id{Bifunctor} \Ax{<} \=\Id{Type} \Ax{\rightarrow} \Id{Functor}\\
\>\> \{\VARS \=\Id{a}, \Id{b}, \Id{c}, \Id{d} \Ax{:} \Id{Type}; \Id{F} \Ax{:} \Id{Bifunctor}; \Id{f} \Ax{:} \=\Id{a} \Ax{\rightarrow} \Id{b}; \\
\>\>\> \Id{g} \Ax{:} \=\Id{b} \Ax{\rightarrow} \Id{c}; \Id{h} \Ax{:} \=\Id{c} \Ax{\rightarrow} \Id{d}\\
\>\> \OP \=\Id{parmap} \Ax{:} \=(\=\Id{a} \Ax{\rightarrow} \Id{b}) \Ax{\rightarrow} \=\Id{F} \Id{a} \Id{d} \Ax{\rightarrow} \=\Id{F} \Id{b} \Id{d}\\
\>\> \Ax{\bullet} \=\Id{parmap} \Id{id} \Ax{=} (\=\Id{id} \Ax{:} \=\Id{F} \Id{a} \Id{d} \Ax{\rightarrow} \=\Id{F} \Id{a} \Id{d})\\
\>\> \Ax{\bullet} \=(\=\Id{parmap} (\=\Id{g} \Id{comp} \Id{f}) \Ax{:} \=\Id{F} \Id{a} \Id{d} \Ax{\rightarrow} \=\Id{F} \Id{c} \Id{d}) \\
\>\>\> \Ax{=} \=\Id{parmap} \Id{g} \Id{comp} \=\Id{parmap} \Id{f};\\
\>\> \}\\
\> \Ax{\bullet} \=(\=\Id{parmap} \Id{f} \Id{comp} \=\Id{map} \Id{h} \Ax{:} \=\Id{F} \Id{a} \Id{c} \Ax{\rightarrow} \=\Id{F} \Id{b} \Id{d}) \\
\>\> \Ax{=} \=\Id{map} \Id{h} \Id{comp} \=\Id{parmap} \Id{f};\\
\KW{end}\\
\\
\SPEC \=\SIdIndex{PolyFunctors} \Ax{=}\\
\> \SId{Functor}\\
\THEN \=\CLASS \=\Id{PolyFunctor} \Ax{<} \Id{Functor}\\
\> \CLASSES \=\Id{PolyBifunctor} \Ax{<} \=\Id{Type} \Ax{\rightarrow} \Id{PolyFunctor};\\
\>\> \Id{PolyBifunctor} \Ax{<} \Id{Bifunctor}\\
\> \VARS \=\Id{F}, \Id{G} \Ax{:} \Id{PolyFunctor}; \Id{H}, \Id{K} \Ax{:} \Id{PolyBifunctor}; \=\Id{a}, \Id{b}, \Id{c} \Ax{:} \Id{Type}\\
\> \TYPE \=\Id{Sum} \=\Id{b} \Id{c} \Ax{::=} \=\Id{inl} \Id{b} \AltBar{} \Id{inr} \Id{c}\\
\> \VARS \=\Id{f} \Ax{:} \=\Id{b} \Ax{\rightarrow?} \Id{a}; \Id{g} \Ax{:} \=\Id{c} \Ax{\rightarrow?} \Id{a}; \Id{h} \Ax{:} \=\Id{Sum} \Id{b} \Id{c} \Ax{\rightarrow?} \Id{a}\\
\> \OP \=\Id{sumcase} \Ax{:} \=(\=\Id{b} \Ax{\rightarrow?} \Id{a}) \Ax{\rightarrow} \=(\=\Id{c} \Ax{\rightarrow?} \Id{a}) \Ax{\rightarrow} \=\Id{Sum} \Id{b} \Id{c} \Ax{\rightarrow?} \Id{a}\\
\> \Ax{\bullet} \=\Id{h} \Ax{=} \=\Id{sumcase} \Id{f} \Id{g} \\
\>\> \Ax{\Leftrightarrow} \=\Ax{\forall} \Id{x} \Ax{:} \Id{b}; \Id{y} \Ax{:} \Id{c} \Ax{\bullet} \=\Id{h} (\=\Id{inl} \Id{x}) \Ax{=} \=\Id{f} \Id{x} \Ax{\wedge} \=\Id{h} (\=\Id{inr} \Id{y}) \Ax{=} \=\Id{g} \Id{y};\\
\> \TYPES \=\Id{Fst} \Id{a} \Id{b} \Id{\Ax{:}\Ax{=}} \Id{a};\\
\>\> \Id{Snd} \Id{a} \Id{b} \Id{\Ax{:}\Ax{=}} \Id{a};\\
\>\> \Id{Id} \Id{b} \Id{\Ax{:}\Ax{=}} \Id{b};\\
\>\> \Id{ExpF} \Id{F} \Id{a} \Id{b} \Id{\Ax{:}\Ax{=}} \=\Id{a} \Ax{\rightarrow} \=\Id{F} \Id{b};\\
\>\> \Id{ExpBF} \Id{H} \Id{a} \Id{b} \Id{c} \Id{\Ax{:}\Ax{=}} \=\Id{a} \Ax{\rightarrow} \=\Id{H} \Id{b} \Id{c};\\
\>\> \Id{ProdF} \Id{F} \Id{G} \Id{b} \Id{\Ax{:}\Ax{=}} \=\Id{F} \Id{b} \Ax{\times} \=\Id{G} \Id{b};\\
\>\> \Id{ProdBF} \Id{H} \Id{K} \Id{b} \Id{c} \Id{\Ax{:}\Ax{=}} \=\Id{H} \Id{b} \Id{c} \Ax{\times} \=\Id{K} \Id{b} \Id{c};\\
\>\> \Id{SumF} \Id{F} \Id{G} \Id{b} \Id{\Ax{:}\Ax{=}} \=\Id{Sum} (\=\Id{F} \Id{b}) (\=\Id{G} \Id{b});\\
\>\> \Id{SumBF} \Id{H} \Id{K} \Id{b} \Id{c} \Id{\Ax{:}\Ax{=}} \=\Id{Sum} (\=\Id{H} \Id{b} \Id{c}) (\=\Id{K} \Id{b} \Id{c})\\
\> \TYPES \=\Id{Fst} \Id{a}, \Id{Id}, \Id{ExpF} \=\Id{F} \Id{a}, \Id{ProdF} \=\Id{F} \Id{G}, \Id{SumF} \=\Id{F} \Id{G} \\
\>\> \Ax{:} \Id{PolyFunctor};\\
\>\> \Id{Fst}, \Id{Snd}, \Id{ExpBF} \=\Id{H} \Id{a}, \Id{ProdBF} \=\Id{H} \Id{K}, \Id{SumBF} \=\Id{H} \Id{K} \\
\>\> \Ax{:} \Id{PolyBifunctor}\\
\> \VAR \Id{k} \Ax{:} \=\Id{a} \Ax{\rightarrow} \Id{b}\\
\> \Ax{\bullet} \=(\=\Id{map} \Id{k} \Ax{:} \=\Id{SumF} \Id{F} \Id{G} \Id{a} \Ax{\rightarrow} \=\Id{SumF} \Id{F} \Id{G} \Id{b}) \\
\>\> \Ax{=} \=\Id{sumcase} (\=\Id{inl} \Id{comp} \=\Id{map} \Id{k}) (\=\Id{inr} \Id{comp} \=\Id{map} \Id{k})\\
\> \Ax{\bullet} \=(\=\Id{parmap} \Id{k} \Ax{:} \=\Id{SumBF} \Id{H} \Id{K} \Id{a} \Id{c} \Ax{\rightarrow} \=\Id{SumBF} \Id{H} \Id{K} \Id{b} \Id{c}) \\
\>\> \Ax{=} \=\Id{sumcase} (\=\Id{inl} \Id{comp} \=\Id{parmap} \Id{k}) (\=\Id{inr} \Id{comp} \=\Id{parmap} \Id{k})\\
\> \Ax{\bullet} \Id{True};\\
\> {\small{}\KW{\%\%} definitions of map and parmap for the other cases}\\
\KW{end}\\
\\
\SPEC \=\SIdIndex{Algebra} \Ax{=}\\
\> \SId{PolyFunctors}\\
\THEN \=\VARS \=\Id{F} \Ax{:} \Id{Functor}; \=\Id{a}, \Id{b} \Ax{:} \Id{Type}\\
\> \TYPE \=\Id{Alg} \Id{F} \Id{a} \Id{\Ax{:}\Ax{=}} \=\Id{F} \Id{a} \Ax{\rightarrow} \Id{a}\\
\> \OP \=\Ax{\_\_}\Ax{::}\Ax{\_\_}\Ax{->}\Ax{\_\_} \Ax{:} \=\Id{Pred} (\=(\=\Id{a} \Ax{\rightarrow} \Id{b}) \Ax{\times} (\=\Id{Alg} \Id{F} \Id{a}) \Ax{\times} (\=\Id{Alg} \Id{F} \Id{b}))\\
\> \VARS \=\Id{f} \Ax{:} \=\Id{a} \Ax{\rightarrow} \Id{b}; \Id{alpha} \Ax{:} \=\Id{Alg} \Id{F} \Id{a}; \Id{beta} \Ax{:} \=\Id{Alg} \Id{F} \Id{b}\\
\> \Ax{\bullet} \=\Id{f} \Ax{::} \Id{alpha} \Ax{->} \Id{beta} \Ax{\Leftrightarrow} \=\Id{beta} \Id{comp} \=\Id{map} \Id{f} \Ax{=} \=\Id{f} \Id{comp} \Id{alpha};\\
\> \TYPE \=\Id{AlgMor} \=\Id{F} \Id{a} \Id{b} \Ax{=} \\
\>\> \{(\=\Id{f}, \Id{alpha}, \Id{beta}) \Ax{:} \=(\=\Id{a} \Ax{\rightarrow} \Id{b}) \Ax{\times} \Id{Alg} \Id{F} \Id{a} \Ax{\times} \=\Id{Alg} \Id{F} \Id{b} \\
\>\> \Ax{\bullet} \=\Id{f} \Ax{::} \Id{alpha} \Ax{->} \Id{beta}\\
\>\> \}\\
\> \CLASSES \=\Id{DTFunctor} \Ax{<} \Id{Functor};\\
\>\> \Id{PolyFunctor} \Ax{<} \Id{DTFunctor}\\
\>\> \{\VARS \=\Id{F} \Ax{:} \Id{DTFunctor}; \Id{a} \Ax{:} \Id{Type}\\
\>\> \TYPE \Id{InitialCarrier} \Id{F}\\
\>\> \OPS \=\Id{initialAlg} \Ax{:} \=\Id{Alg} \Id{F} (\=\Id{InitialCarrier} \Id{F});\\
\>\>\> \Id{ifold} \Ax{:} \=\Id{Alg} \Id{F} \Id{a} \Ax{\rightarrow} \=\Id{InitialCarrier} \Id{F} \Ax{\rightarrow} \Id{a}\\
\>\> \VARS \=\Id{alpha} \Ax{:} \=\Id{Alg} \Id{F} \Id{a}; \Id{g} \Ax{:} \=\Id{InitialCarrier} \Id{F} \Ax{\rightarrow} \Id{a}\\
\>\> \Ax{\bullet} \=\Id{g} \Ax{::} \Id{initialAlg} \Ax{->} \Id{alpha} \Ax{\Leftrightarrow} \=\Id{g} \Ax{=} \=\Id{ifold} \Id{alpha};\\
\>\> \}\\
\> \VAR \Id{G} \Ax{:} \Id{PolyBifunctor}\\
\> \TYPE \=\Id{ParamDT} \Id{G} \Id{a} \Id{\Ax{:}\Ax{=}} \=\Id{InitialCarrier} (\=\Id{G} \Id{a})\\
\> \TYPE \=\Id{ParamDT} \Id{G} \Ax{:} \Id{DTFunctor}\\
\> \VARS \=\Id{l} \Ax{:} \=\Id{ParamDT} \Id{G} \Id{a}; \Id{b} \Ax{:} \Id{Type}; \Id{f} \Ax{:} \=\Id{a} \Ax{\rightarrow} \Id{b}\\
\> \Ax{\bullet} \=\Id{map} \Id{f} \Id{l} \Ax{=} \=\Id{ifold} (\=\Id{initialAlg} \Id{comp} \=\Id{parmap} \Id{f}) \Id{l};\\
\KW{end}
\end{hetcasl}

